Graphene: Infrastructure Security Posture Analysis with AI-generated Attack Graphs

The rampant occurrence of cybersecurity breaches imposes substantial limitations on the progress of network infrastructures, leading to compromised data, financial losses, potential harm to individuals, and disruptions in essential services. The current security landscape demands the urgent development of a holistic security assessment solution that encompasses vulnerability analysis and investigates the potential exploitation of these vulnerabilities as attack paths. In this paper, we propose Graphene, an advanced system designed to provide a detailed analysis of the security posture of computing infrastructures. Using user-provided information, such as device details and software versions, Graphene performs a comprehensive security assessment. This assessment includes identifying associated vulnerabilities and constructing potential attack graphs that adversaries can exploit. Furthermore, Graphene evaluates the exploitability of these attack paths and quantifies the overall security posture through a scoring mechanism. The system takes a holistic approach by analyzing security layers encompassing hardware, system, network, and cryptography. Furthermore, Graphene delves into the interconnections between these layers, exploring how vulnerabilities in one layer can be leveraged to exploit vulnerabilities in others. In this paper, we present the end-to-end pipeline implemented in Graphene, showcasing the systematic approach adopted for conducting this thorough security analysis.

==> Archive/Dashboard.tex <==
\subsection{Dashboard}

The dashboard serves as the front-end user interface of the \sysname system. As \sysname breaks down the security posture analysis of a given infrastructure, the envisioned users of the interface are security officers and subject matter experts of the individual layers. 

Figure~\ref{fig:\sysname_dashboard_gen} shows \sysname's front-end dashboard interface snapshot. The figure showcases a spider graph delineating the top three identified vulnerabilities and subsequently outlines the top three high-severity paths. Additionally, a table excerpt is presented, detailing identified vulnerabilities along with their corresponding extracted pre- and post-conditions.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.5\textwidth]{Figures/attack-graph-example.pdf}
\caption{An example of a generated attack graph with two intermediate nodes; the first node is an ML layer CVE, and the second is a hardware \& system CVE.}
\label{fig:crypto-graph-gen}
\end{figure}

The user is additionally able to introduce new nodes in the graph (i.e., new CVEs) and modify or delete existing ones. Such functionality is needed as often online resources are not immediately updated once a certain vulnerability is disclosed. Moreover, the risk, exploitability, and impact scores may not reflect the criticality of the resources in the infrastructure (e.g., overestimated or underestimated scores). Thus, \sysname allows users to change those scores.

Once the user makes such changes, the dashboard communicates the request to the back end, where a change-impact analysis occurs. The results are returned to the dashboard, which gets immediately updated.

\begin{figure*}[htbp]
\centerline{\includegraphics[width=1.5\columnwidth]{Figures/dashboard_gen.png}}
\caption{
A small snapshot of \sysname's front-end dashboard interface. 
\label{fig:\sysname_dashboard_gen}
}
\end{figure*}

% Finally, the dashboard showcases analytics generated from the back-end processing. Among many things, the analytics show the most high-risk vulnerabilities and paths that an attacker may potentially exploit. The analytics are computed and shown separately for the cumulative attack graph and each of the layered attack graphs.

The dashboard also illustrates the generated attack graphs for the given infrastructure for the different layers. For example, figure~\ref{fig:crypto-graph-gen} shows an example of a multi-layer attack graph. The first CVE node is classified under the ML layer, whereas the second CVE is under the hardware and systems area.

The dashboard also provides visual representations of the generated attack graphs pertaining to distinct layers within the designated infrastructure. For instance, Figure~\ref{fig:crypto-graph-gen}, illustrates a multi-layer attack graph generated by \sysname. In this illustration, the initial CVE node is categorized within the Machine Learning (ML) layer, while the subsequent CVE node is categorized within the domain of hardware and systems.
% The generated attack graph may be overly dense. However, due to \sysname's fine-grained approach, one can see the reductions of the cumulative graph to a specific security layer graph. Figure~\ref{fig:crypto-graph-gen} shows a cryptography layer attack graph reduced from the cumulative attack graph.
